Diffusion-based Time Series Data Imputation for Microsoft 365

Reliability is extremely important for large-scale cloud systems like Microsoft 365. Cloud failures such as disk failure, node failure, etc. threaten service reliability, resulting in online service interruptions and economic loss. Existing works focus on predicting cloud failures and proactively taking action before failures happen. However, they suffer from poor data quality like data missing in model training and prediction, which limits the performance. In this paper, we focus on enhancing data quality through data imputation by the proposed Diffusion+, a sample-efficient diffusion model, to impute the missing data efficiently based on the observed data. Our experiments and application practice show that our model contributes to improving the performance of the downstream failure prediction task.

==> results_note.tex <==

RMSE           Ali (10,50,90)                         

Baseline1   
Baseline2
Baseline3
CSDI           0.523684342228123    0.38972270073102744 
Ours
------------------------------------------------------
RMSE           Back (10,50,90)                          
Baseline1   
Baseline2
Baseline3
CSDI          
Ours

-----------------------------------------------------------
RMSE           office (10,50,90)                          
Baseline1   
Baseline2
Baseline3
CSDI           
Ours

% =======================================================

MAE           Ali  (10,50,90)                       

Baseline1   
Baseline2
Baseline3
CSDI       0.09871270748656961          0.05649740355769146 
Ours

--------------------------------------------------------------
MAE           Back  (10,50,90)                       

Baseline1   
Baseline2
Baseline3
CSDI  
Ours

--------------------------------------------------------------
MAE           Office  (10,50,90)         

Baseline1   
Baseline2
Baseline3
CSDI  
Ours

% ==================================================================


CRPS           Ali  (10,50,90)                       

Baseline1   
Baseline2
Baseline3
CSDI         0.39695526424207184        0.21094026063617907
Ours
--------------------------------------------
CRPS           Back  (10,50,90)                   

Baseline1   
Baseline2
Baseline3
CSDI                 
Ours

--------------------------------------------
CRPS           Office  (10,50,90)                       
Baseline1   
Baseline2
Baseline3
CSDI                 
Ours

% ===================================================================================================

% Failure prediction 
% Office m365            
% zero-padding + LSTM       Best top_acc: 57.00%, F1: 58.55%, Precision: 64.06% Recall: 53.91%
% zero-padding + NTAM       Best top_acc: 56.58%, F1: 58.49%, Precision: 62.53% Recall: 54.94%
% zero-padding + TCNN       Best top_acc: 57.41%, F1: 59.95%, Precision: 66.58% Recall: 54.53%



% We have run our Diffusion\textsuperscript{\plus} model on Microsoft 365, which contains millions of disks. In particular, our model takes effect in the data process phase of the current disk failure prediction pipeline~\cite{liu2022multi}. The SMART data is first collected by a data collection service, transferred by a distributed streaming tool, and stored in Azure. Then, our model imputes missing data before sending it to the feature engineering of the downstream prediction tasks. 
% We conduct A/B testing to measure the effectiveness of our model and its contribution to service reliability. We monitor the reduction of virtual machine (VM) interruptions by taking proactive failure mitigation based on the prediction. Compared with the original data process phase without Diffusion\textsuperscript{\plus}, the interruptions have reduced the VM interruptions and enhanced the service reliability to avoid potential financial loss.

==> table.tex <==
% 0.1 missing
% zero: RMSE: 1.0505382648103325
% zero: MAE: 0.3264232631593795
% forward: RMSE: 0.6080635964071086
% forward: MAE: 0.06194566453769431
% linear: RMSE: 0.5151277369869853
% linear: MAE: 0.05092894456956037

% zero: RMSE: 1.1230596623662292
% zero: MAE: 0.3259957617265481
% forward: RMSE: 0.6560203702519839
% forward: MAE: 0.0626199758004481
% linear: RMSE: 0.5953726202659071
% linear: MAE: 0.05158391188042259

% 0.5 missing
% zero: RMSE: 0.9741660621472898
% zero: MAE: 0.32554792110283626
% forward: RMSE: 0.697311389118978
% forward: MAE: 0.07089595882917725
% linear: RMSE: 0.5966432957611456
% linear: MAE: 0.05861165163087327

% zero: RMSE: 1.0287873804239358
% zero: MAE: 0.32514098296386384
% forward: RMSE: 0.6712703603039996
% forward: MAE: 0.07097888558557511
% linear: RMSE: 0.5383261240102145
% linear: MAE: 0.058878650727574366

% 0.9 missing
% zero: RMSE: 0.9660700943104003
% zero: MAE: 0.32547260991120636
% forward: RMSE: 0.7960388088546522
% forward: MAE: 0.11219788063582356
% linear: RMSE: 1.4372490735052148
% linear: MAE: 0.1099120348850012

% zero: RMSE: 1.0084980274306021
% zero: MAE: 0.32503418995626204
% forward: RMSE: 0.7481601673349341
% forward: MAE: 0.11170291356713719
% linear: RMSE: 0.9526839547491149
% linear: MAE: 0.108731061585337

0.1missing
zero: RMSE: 1.1039722777783658
zero: MAE: 0.4290026948190121
forward: RMSE: 0.6697161326670178
forward: MAE: 0.04734388087025184
linear: RMSE: 0.7028815063534825
linear: MAE: 0.038612382619633345

tf.Tensor(0.33882046, shape=(), dtype=float32)
tf.Tensor(1.0992626, shape=(), dtype=float32)
tf.Tensor(1.6772678, shape=(), dtype=float32)
tf.Tensor(2.370409, shape=(), dtype=float32)
tf.Tensor(3.0639768, shape=(), dtype=float32)
NLL miss: 1.1524
MSE miss: 0.4641
MAE miss: 0.0517
CRPS: 0.6128
AUROC: 0.7033
AUPRC: 0.2635

0.5missing
zero: RMSE: 1.0658290205796201
zero: MAE: 0.4290296879083303
forward: RMSE: 0.7551082234486837
forward: MAE: 0.05675866818050711
linear: RMSE: 0.8715805238520099
linear: MAE: 0.044513963023488416

tf.Tensor(0.33933544, shape=(), dtype=float32)
tf.Tensor(1.1022155, shape=(), dtype=float32)
tf.Tensor(1.6846185, shape=(), dtype=float32)
tf.Tensor(2.382601, shape=(), dtype=float32)
tf.Tensor(3.0794494, shape=(), dtype=float32)
NLL miss: 1.1429
MSE miss: 0.4735
MAE miss: 0.0536
CRPS: 0.6159
AUROC: 0.6963
AUPRC: 0.2235



0.9 missing
zero: RMSE: 1.0550702681532498
zero: MAE: 0.42895955651976636
forward: RMSE: 0.9332765528288183
forward: MAE: 0.11059606711928996
linear: RMSE: 1.139474739898775
linear: MAE: 0.0802261364179294

zero:
lstm:
Final best top_acc: 54.26% At epoch 10, F1: 55.06% At epoch 9, Precision: 55.89% Recall: 54.26%, Auc: 79.87%, PR: 34.15%
trans:
Final best top_acc: 54.04% At epoch 17, F1: 54.79% At epoch 17, Precision: 60.60% Recall: 50.00%, Auc: 81.28%, PR: 37.09%
tcnn:
Final best top_acc: 54.04% At epoch 3, F1: 56.32% At epoch 15, Precision: 68.15% Recall: 47.98%, Auc: 82.34%, PR: 45.20%

forward:
lstm:
Final best top_acc: 50.67% At epoch 29, F1: 54.05% At epoch 31, Precision: 64.69% Recall: 46.41%, Auc: 83.11%, PR: 41.35%
trans:
Final best top_acc: 51.35% At epoch 3, F1: 54.75% At epoch 8, Precision: 62.97% Recall: 48.43%, Auc: 82.19%, PR: 34.87%
tcnn:
Final best top_acc: 50.67% At epoch 3, F1: 54.38% At epoch 3, Precision: 63.94% Recall: 47.31%, Auc: 82.92%, PR: 43.11%

linear:
lstm:
Final best top_acc: 51.57% At epoch 28, F1: 54.79% At epoch 30, Precision: 61.62% Recall: 49.33%, Auc: 83.34%, PR: 38.43%
trans:
Final best top_acc: 51.12% At epoch 1, F1: 54.57% At epoch 3, Precision: 62.87% Recall: 48.21%, Auc: 82.01%, PR: 33.72%
tcnn:
Final best top_acc: 50.45% At epoch 4, F1: 54.81% At epoch 22, Precision: 66.45% Recall: 46.64%, Auc: 80.68%, PR: 37.38%

imputation method zero_imputation + prediction lstm
Best top_acc: 54.04%, F1: 54.81%, Precision: 60.00% Recall: 50.45% 
imputation method forward_imputation + prediction lstm
Best top_acc: 58.55%, F1: 59.80%, Precision: 61.35% Recall: 58.33% 
imputation method linear_interpolation + prediction lstm
Best top_acc: 55.26%, F1: 57.50%, Precision: 64.05% Recall: 52.16% 
imputation method zero_imputation + prediction tcnn
Best top_acc: 54.04%, F1: 56.65%, Precision: 62.84% Recall: 51.57% 
imputation method forward_imputation + prediction tcnn
Best top_acc: 58.76%, F1: 60.48%, Precision: 64.34% Recall: 57.05% 
imputation method linear_interpolation + prediction tcnn
Best top_acc: 55.26%, F1: 57.89%, Precision: 65.04% Recall: 52.16% 
imputation method zero_imputation + prediction ntam
Best top_acc: 56.16%, F1: 58.46%, Precision: 62.64% Recall: 54.79% 
imputation method forward_imputation + prediction ntam
Best top_acc: 53.71%, F1: 55.37%, Precision: 61.05% Recall: 50.66% 
imputation method linear_interpolation + prediction ntam
Best top_acc: 56.50%, F1: 57.77%, Precision: 59.82% Recall: 55.86% 


diff:
lstm:
Final best top_acc: 59.37% At epoch:68, F1: 60.60% At epoch 72, Precision: 66.75% Recall: 55.49%, Auc: 97.83%, PR: 47.82%

trans:
Final best top_acc: 59.49% At epoch:72, F1: 62.18% At epoch 78, Precision: 74.05% Recall: 53.59%, Auc: 98.07%, PR: 62.37%

tcnn:
Final best top_acc: 58.44% At epoch:18, F1: 60.03% At epoch 18, Precision: 79.24% Recall: 48.31%, Auc: 98.31%, PR: 66.12%

% We have run our Diffusion\textsuperscript{\plus} model on Microsoft 365, which contains millions of disks. In particular, our model takes effect in the data process phase of the current disk failure prediction pipeline~\cite{liu2022multi}. The SMART data is first collected by a data collection service, transferred by a distributed streaming tool, and stored in Azure. Then, our model imputes missing data before sending it to the feature engineering of the downstream prediction tasks. 
% We conduct A/B testing to measure the effectiveness of our model and its contribution to service reliability. We monitor the reduction of virtual machine (VM) interruptions by taking proactive failure mitigation based on the prediction. Compared with the original data process phase without Diffusion\textsuperscript{\plus}, the interruptions have reduced the VM interruptions and enhanced the service reliability to avoid potential financial loss.
